How to Save My Gas Fees: Understanding and Detecting Real-world Gas Issues in Solidity Programs

The execution of smart contracts on Ethereum, a public blockchain system, incurs a fee called gas fee for its computation and data storage. When programmers develop smart contracts (e.g., in the Solidity programming language), they could unknowingly write code snippets that unnecessarily cause more gas fees. These issues, or what we call gas wastes, can lead to significant monetary losses for users. This paper takes the initiative in helping Ethereum users reduce their gas fees in two key steps. First, we conduct an empirical study on gas wastes in open-source Solidity programs and Ethereum transaction traces. Second, to validate our study findings, we develop a static tool called PeCatch to effectively detect gas wastes in Solidity programs, and manually examine the Solidity compiler's code to pinpoint implementation errors causing gas wastes. Overall, we make 11 insights and four suggestions, which can foster future tool development and programmer awareness, and fixing our detected bugs can save $0.76 million in gas fees daily.

==> tables/tbl-gas-impact.tex <==
\begin{table}[t]
\centering
\footnotesize
{
\mycaption{tab:gas-impact}
{Gas impact of patterns.}
{
\textit{(Column total gas cost represents the total gas usage of the pattern as described in section C. Column saving of one execution represents the gas saving of one execution of the example contract which can be found at~\cite{gas-impact:url})}}
\begin{tabular}{|l|c|c|c|}
\hline
{\textbf{pattern}}   & {\textbf{total gas cost}} & {\textbf{percentage}} & {\textbf{saving per execution}}\\

%\midrule
\hline
\hline

no side effect  & 34.4B & 4.5\% & - \\ \hline
\&\& in if  & 1.7B  & 0.22\% & 23,8 \\ \hline
allocation in loop  & 74.5B & 79.7B & 15X-15 \\ \hline
zero to one  &  &  &  \\ \hline
Repetitive sload & 9.9B & 1.3\% & 266 \\ \hline
Repetitive sstore & 299.1M & 0.04\% & - \\ \hline
Repetitive memory read & 927.1M & 0.12\% & - \\ \hline

\hline
\end{tabular}
% \vspace{-0.25in}
}
\end{table}

==> tables/tbl-transactions.tex <==
\begin{table}[t]
\centering
\footnotesize
{
\mycaption{tab:transaction}
{Transaction data every day.}
{
\textit{(The gas used and gas fee represent the execution cost of successful transactions.)}}
\begin{tabular}{|l|c|c|c|}
\hline
        & {\textbf{min}} & {\textbf{max}} & {\textbf{average}}\\

%\midrule
\hline
\hline

block  & 7112 & 7135 & 7123.4 \\ \hline
successful transaction  & 988840  & 1118454 & 1062930.7\\ \hline
gas used  & 74.5B & 79.7B & 76.6B \\ \hline
gas fee  & \$15.5M & \$16.6M & \$16.0M \\


\hline
\end{tabular}
% \vspace{-0.25in}
}
\end{table}
